SoK: A cloudy view on trust relationships of CVMs -- How Confidential Virtual Machines are falling short in Public Cloud

Confidential computing in the public cloud intends to safeguard workload privacy while outsourcing infrastructure management to a cloud provider. This is achieved by executing customer workloads within so called Trusted Execution Environments (TEEs), such as Confidential Virtual Machines (CVMs), which protect them from unauthorized access by cloud administrators and privileged system software. At the core of confidential computing lies remote attestation -- a mechanism that enables workload owners to verify the initial state of their workload and furthermore authenticate the underlying hardware. hile this represents a significant advancement in cloud security, this SoK critically examines the confidential computing offerings of market-leading cloud providers to assess whether they genuinely adhere to its core principles. We develop a taxonomy based on carefully selected criteria to systematically evaluate these offerings, enabling us to analyse the components responsible for remote attestation, the evidence provided at each stage, the extent of cloud provider influence and whether this undermines the threat model of confidential computing. Specifically, we investigate how CVMs are deployed in the public cloud infrastructures, the extent to which customers can request and verify attestation evidence, and their ability to define and enforce configuration and attestation requirements. This analysis provides insight into whether confidential computing guarantees -- namely confidentiality and integrity -- are genuinely upheld. Our findings reveal that all major cloud providers retain control over critical parts of the trusted software stack and, in some cases, intervene in the standard remote attestation process. This directly contradicts their claims of delivering confidential computing, as the model fundamentally excludes the cloud provider from the set of trusted entities.

==> evaluation/aws.tex <==
On AWS, Confidential Computing offerings revolve around AMD SEV-SNP. Bare metal servers (BMS) and VMs (EC2 instances, in this case) are both supported. As BMS offerings by design do not enable to reap the benefits of hyperscalers as effectively as VM offerings, the latter will be the main consideration. Currently, AWS does not offer nested virtualization.

(1) Can the TCB be configured?

The software running on the AMD SP cannot be influenced by the customer nor has the customer any choice in firmware provided for the CVM. Building upon this, the customer is able to select or even provide an OS image. Unfortunately, said image is restricted to the Amazon Machine Image (AMI) format which ensures compatibility with the AWS ecosystem. AMIs can only be derived from other AMIs or through importing a VM image by utilizing a closed-source utility provided by AWS. Only these imported images can be exported (through the utility) again. Therefore, it is currently impossible to review which differences AMIs have to other VM images, which raises security concerns. With the images being essentially impossible to export in a useful way, reference measurements can at best be gathered on AWS infrastructure as even just receiving the AMI in a file format proves to be impossible for a customer.

(2) Can it be validated?

Can we retrieve and individualize an attestation report?
Yes, it is possible to supply 64 bytes of user-chosen data that will be embedded into the attestation report.

(1) Who owns the different layers/components used to configure
and produce the report?

AMD owns the software running on the AMD processor which they produced and maintains the key infrastructure. The CSP physically owns the hardware involved and provides parts of the software required to run the CVM, i.e. guest firmware and image tools.

(2) Are these components open source and can be validated or
closed and what entity do we have to trust in that case?

UEFI firmware is supplied by AWS. It is open source and can be reproducibly built. 

(3) Who is the root of trust for the report? Is there a trust chain
of different entities? (e.g., hardware vendor, cloud provider
etc.)

The root of trust is the AMD SP and more abstractly speaking the AMD root key. \textit{In particular, its derivations, the Versioned Chip Endorsement Keys (VCEK) and in a CSP-context the Version Loaded Endorsement Key (VLEK), which are provisioned by AMD for that particular chip or CSP, respectively, are of particular note here.} AWS utilizes VLEKs \textit{which are generated and managed by AMD with CSPs having specific seeds}.

(4) Can the customer provision a different root of trust or trust
chain?

The customer cannot influence the root of trust selection.

(5) What exactly is covered by the measurement of the attesta-
tion report? Example: HW/SW of CPU provider, customer
code/data, cloud provider SW/HW

The AMD SEV-SNP attestation report covers the software running on the AMD SP and the guest firmware as the initial memory pages are measured. This basic report does not cover beyond that, so that attestation of the user kernel, OS and applications/data must be achieved through additional means.

(6) Is there additional data that can be included/linked into the
report? Example: Data provided by the TEE protected SW,
additional data provided during setup (customer, developer
and provider)

\textit{The AMD SEV-SNP attestation report provides the option to include 64 bytes of data. Utilizing this, it is possible to provide a nonce to guarantee report freshness or, e.g, link another attestation mechanism such as a TPM by including a hash of its public key in the attestation report. It is important to keep the size limitation and the non-standardisation in mind as conflicts may arise when using publically available tools such as Constellation. }

(7) Are the communication paths to create an attestation re-
port integrity-protected and secure? Which components are
involved?

The AMD SP is exposed as a device under \texttt{/dev/snp-guest} inside the CVM. By, e.g. utilizing the VirTEE \texttt{snpguest} utility, it is therefore possible to communicate with the AMD SP from inside the CVM. An attestation report can be requested and output to a file. While it is already possible to also check the validity of the signature and policy compliance inside the CVM, it is more prudent to forward this attestation report to the respective verifier in the context of remote attestation. The exact means of this export is left for the customer to implement.

Furthermore, AWS also offers Nitro Enclaves. Their main focus is to outsource sensitive computation from the guest themselves to an enclave in order to protect the guest from themselves, which is a concept similarly found in Intel SGX. Unfortunately, as these Nitro Enclaves are managed and enforced by the Nitro Hypervisor, i.e. AWS, they cannot be trusted if the CSP as a whole is by definition not trusted in a Confidential Computing context.

==> evaluation/aws2.tex <==
On AWS, Confidential Computing offerings revolve around AMD SEV-SNP. Bare metal servers (BMS) and virtual machines (EC2 instances, in this case) are both supported. As BMS offerings by design do not enable one to reap the benefits of hyperscalers as effectively as VM offerings, the latter will be the main consideration. 
VMs with SEV-SNP support can currently only be launched in the Ireland and Ohio regions. This can be achieved by enabling AMD SEV-SNP in the VM launch configuration. In addition, a customer must select a VM image. These images are in Amazon Machine Image (AMI) format. There are currently two documented ways to generate an AMI: importing a VM image from another solution like VMWare or deriving one from an already existing one. The latter is preferred. Both approaches utilize currently closed-source AWS tools. Currently, there is no documented way for a customer to explicitly download an AMI. AMIs imported from another VM solution can be exported, but this will output the image in that specific VM solution format and the process uses closed-source AWS utilities once again. Therefore, the customer cannot independently perform measurements on the AMI. During VM launch configuration, it is also possible to select a specific kernel and RAM disk, which differs from the default preference of the AMI in question, but the lists are populated by AWS. Alternatively, a user could launch a VM with a base image, make the necessary adjustments to the kernel, the RAM disk, and other potential subjects of interest such as OS configuration and installed packages. Then, the user could create a new AMI based on this specific VM, and the preferred values would be reflected in any VM based on this specific AMI.
The UEFI firmware running beneath the VM image is provided by AWS. It is open source and can be built reproducibly. As the firmware is measured by AMD SEV-SNP during launch, it is therefore possible for a customer to ensure that this specific firmware is running. It is currently not possible for a customer to select other or provide their own firmware.
The AMD SP is exposed to the guest VM under \texttt{/sev/snp-guest}. Therefore, the guest VM can communicate with it from inside. An attestation report can be requested and output to a file. Although it is already possible check the validity of the signature and policy compliance from inside the CVM, it is more prudent to forward this attestation report to the respective verifier in the context of remote attestation. The exact means of this export is on the customer to implement.
The attestation report is signed by a Versioned Loaded Endorsement Key (VLEK) instead of the commonly encountered VCEK. The VLEK also utilizes the same SVNs as the VCEK to integrate the TCB version numbers into its key generation function, but the VLEK uses a CSP specific secret as a seed for it rather than a secret unique to the chip which is stored in burnt-in fuses. The CSP specific secret is managed by AMD and CSPs can only request wrapped VLEKs from AMD which can only be unwrapped inside the according AMD SPs. 
The attestation report itself only covers the AMD SP specific TCB

Currently, AWS does not offer nested virtualization.

==> evaluation/azure.tex <==
Azure offers confidential computing on the basis of Intel SGX as well as AMD-SEV-SNP, providing both in a VM as well as a container setting.

While Intel SGX -capable VMs and Azure Kubernetes Service (AKS) with added Intel SGX confidential computing VM nodes come with pre-installed Intel SGX DCAP driver, hence allowing direct attestation of enclaves, e.g. via the used framework, such as SCONE CAS, AMD-SEV-SNP -capable VMs, called Confidential VMs (CVMs) in Azure-terms are more problematic.
% https://learn.microsoft.com/en-us/azure/confidential-computing/confidential-nodes-aks-overview
CVMs come with a virtual TPM (vTPM), whose implementation is unfortunately not public, and which therefore cannot be independently attested.
Microsoft claims that they employ an automated system called Azure Attestation, that verifies each CVM upon startup against a user-specifiable Attestation Policy, but this does not expose any checks to tenants and also does not help with operator exclusion.
To attest a CVM without reliance on this system, they offer so-called “guest attestation”, which comes in two flavours. Either one uses Microsoft Azure Attestation (MAA) with the open-source \texttt{azguest} dynamic library to handle communication to the MAA service, or retrieves the hardware report from the vTPM directly and validates it against the VCEK using e.g. VirTEE \texttt{sevtool}.

The Microsoft Azure Attestation (MAA) service is implemented in an SGX enclave.
It abstracts over attestation of different CC technologies and provides attestation tokens, i.e. special JSON Web Tokens (JWTs) with claims related to attestation.
Such a JWT is signed by a private key which has an enclosed Intel SGX report in an X.502 extension. The contained \texttt{MRENCLAVE} can be compared against an Azure-published value, but since the MAA implementation is not open-source, it is impossible to convince oneself independently of its correct/benign implementation or even to reproduce the measurement.

Although directly fetching the hardware report from the vTPM eliminates the need to trust MAA, it is not possible to ensure the freshness of this report as it is generated once on VM startup and then stored in the vTPM. Also, the firmware within CVMs, referred to as Hardware Compatibility Layer (HCL) by Azure, remains in the TCB and cannot be inspected by tenants. It stands to reason that the vTPM implementation is part of the HCL, but this is not documented.
% https://learn.microsoft.com/en-us/azure/confidential-computing/confidential-vm-overview
% https://github.com/Azure/confidential-computing-cvm-guest-attestation/blob/main/PlatformGuestAttestation-APIdoc.pdf
% https://github.com/Azure/confidential-computing-cvm-guest-attestation/blob/main/cvm-guest-attestation.md

Next to CVMs, Azure offers AMD-SEV-SNP also in Azure Container Instances (AKI). This applies Parma, a framework to extend the integrity measurement from an SEV  launch digest to a container runtime. On AKI, containers are organized in groups, each with its own Confidential Computing Enforcement (CCE) policy. The CCE policies are specified in the Rego policy language and incorporated into the firmware, s.t. the launch digest covers them.

The Azure-CLI allows tenants to deploy their Azure infrastructure declaratively by using Azure Resource Manager (ARM) templates. It integrates with a “confcomp” extension to facilitate confidential containers on AKI.
For instance, \texttt{az confcom acipolicygen -a ./template.json}
will modify the given ARM template by inserting the base64-encoded Rego CCE policy which it automatically generates from the template.
However, it currently is available as preview version only.

There are two open-source sidecars to be deployed alongside a confidential AKI container:
Secure Key Release (SKR) sidecar can provision keys from either Azure Key Vault (AKV) or a managed Hardware Security Module (mHSM), presenting attestation tokens for the container group in the process. AKV requires trust in Azure, as it is neither open-source nor can it be attested. Similarly, an mHSM cannot be attested and the HSM vendor needs to be trusted.
Additionally there is Encrypted Filesystem sidecar, which uses SKR to interact with AKV and decrypt a volume.
Furthermore, the SKR offers an endpoint for retrieval of the AMD-SEV-SNP attestation report or an MAA attestation JWT. 

Although the “confcomp” CLI-extension and sidecar containers are open-source, one cannot directly check the exact software running on the underlying AMD-SEV-SNP -based CVMs of the container group in ACI.
% https://learn.microsoft.com/en-us/azure/container-instances/container-instances-confidential-overview
% https://github.com/microsoft/confidential-sidecar-containers
% https://github.com/Azure/azure-cli-extensions/blob/main/src/confcom/azext_confcom/README.md
% https://github.com/microsoft/confidential-container-demos/tree/main/hello-world/ACI

\subsection{AMD SEV-SNP CVM Confidential Container Group - only preview version?}

Azure furthermore provides the possibility to launch Confidential Container Groups on Azure Container Instances (ACI) using AMD SEV-SNP.

It is possible to use MAA 


As for CVMs, the Owner configures the target by using an Arm template. The configuration of a Container Group additionally allows to specify execution policies, based on the Parma architecture by Johnson et al.~\cite{johnson2024confidential}. These policies are configured using the confcomp extension\footnote{https://github.com/Azure/azure-cli-extensions/blob/main/src/confcom/azext\_confcom/README.md, retrieved on 29/01/2025} and can be verified. The policies use dm-verity for linking image layers.

The guest is fully enlightened. Therefore, they are able to retrieve fresh attestation reports directly from hardware. However, we were not able to fetch the VCEK from hardware as well and therefore had to retrieve it from the Azure service THIM. Azure offers an open-source attestation sidecar container\footnote{https://github.com/microsoft/confidential-sidecar-containers/tree/main/cmd/attestation-container, retrieved on 29/01/2025} alternatively.


\paragraph{Identity Establishment}

The identity establishment is similar to CVMs. It is not possible to provide identity data at boot time. However, it is possible to provide custom report data on request of an attestation report, which can be used for identity data.

\paragraph{Metrics}



The Owner of the Container Group is able to configure the guest via execution policies. The SHA-256 digest of the policy is contained in the attestation report via the host data attribute and immutable. 

As it is possible to provide custom data on request of an attestation report, the guest is able to link a public key to the container group and ensure freshness by providing a nonce.


\paragraph{TCB}


\subsection{Intel SGX}

Similar to AMD CVMs, Intel SGX enclaves are deployed via Arm templates. 
Attestation is possible using either EPID or DCAP.

When using DCAP, the user is expected to install Azure's DCAP client as quoting data provider plugin, which handles fetching artifacts from an Azure caching service. Intel CAs are the root authority of all data.

Various tools can be used for the development of enclave applications. Possible open source options are the following:
\begin{enumerate}
    \item Open Enclave SDK or EGo SDK 
    \item Intel SGX SDK
    \item Confidential Constortium Framework
\end{enumerate}

\paragraph{Identity Establishment}

\paragraph{Metrics}

tbd.

\paragraph{Trusted Computing Base}

tbd.

==> evaluation/google_confidential_space.tex <==
\subsubsection{Confidential Space}

\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{figures/google-container.pdf}
    \caption{\ac{GCP} \ac{SEV} Container: Architecture.}
    \label{fig:google-container}
\end{figure}

GCP provides confidential containers under the name of Confidential Space running on AMD \ac{SEV}.
Intel \ac{TDX} is available as well, but currently in preview version and for that reason not considered.
In the following, we analyse the AMD \ac{SEV} offering, although \ac{SEV} does not provide integrity protection~\cite{menetrey2022attestation}. 
We still regard the analysis as essential, as future \ac{GCP} confidential container architectures will probably rely on similar attestation architectures.

A Confidential Space system consists of three core components:
\begin{itemize}
    \item A protected resource, a managed cloud resource supporting Workload Identity Federation.
    \item A workload, which is a containerised image that processes the protected resource.
    The container is to be deployed on a special OS called Confidential Space image~\cite{GoogleConfSpaceImage}, which runs in an AMD \ac{SEV} \ac{CVM}.
    The Confidential Space image is closed source and provided by GCP, based on the open source ChromiumOS~\cite{ChromiumOS}.
    \item  (GCA), an open source attestation service~\cite{GoogleCloudAttestation} hosted on GCP, which functions as the verifier. This has to be trusted implicitly as it cannot be attested.
    \jana{Is it really open source? You provided the link for go-tpm-tools, which is only used by GCP I guess. Would use this reference~\cite{GoogleCloudAttestationService} instead.}
\end{itemize}

Relevant for attestation are the following components, as depicted in Figure~\ref{fig:google-container}:
\begin{itemize}
    \item the \ac{CVM}, which is to be attested;
    \item a vTPM, running outside of the \ac{CVM} which is utilised for measured boot and runtime measurements;
    \item GCA, the verifier used for attestation. The guest is not enlightened, attestation therefore relies on GCA.
\end{itemize}

Before resource owners (relying parties) execute the processing within the workload, the status of the workload has to be attested.
To achieve that, they initiate an attestation request, with optional nonces, to the GCA service.
The GCA returns an attestation token, including attested attributes and echoed nonces.
The relying parties then verify the attested attributes using self-defined assertion policies.
The assertion policies have three categories:
\begin{itemize}
    \item VM assertions: \ac{CVM} information such as name, ID, region, and hardware model.
    \item Image assertions: Guest OS information such as version and debug flag of the Confidential Space image.
    \item Container assertions: Container information such as image digest or signature, startup commands, and parameters, as well as environment variables. 
\end{itemize}
Once the verification succeeds, they can continue with the actual confidential computing.
However, the attestation is not transparent to the customer and is presumably only implemented in software using the vTPM~\cite{googleContainerAttestation}.

\paragraph{Identity Establishment}

No \ac{HRoT} is participating in attestation.
Instead, a vTPM, running outside of the \ac{CVM}, is used for measured boot, but inaccessible to the customer.
Therefore, it is unclear which identity, if any, is signing the vTPM collected evidence.
No unique target identity is established, as the owner cannot access attestation reports.

\paragraph{Attestation-collateral Metrics}

At loading time, the virtual firmware, the guest OS, and the container are measured.
\jana{which components measures them? I think it's the vTPM.}
\tian{"The vTPM signs (or quotes) these measurements using a certified attestation key that is trusted by Google Cloud Attestation."}
The guest is unable to retrieve the hardware attestation report.

The runtime measurements are conducted by the vTPM, but is not accessible to the relying parties either.
\jana{Not sure if there are any runtime measurements, since we can't access the vTPM.}
\tian{No way to verify that even though they mentioned "extended runtime measurements" in the attestation process.}
Instead, attestation relies on the attestation tokens issued by GCA, which is not attestable.


\jana{
previous text:
At loading time, the \ac{CVM}, the guest OS (Confidential Space image), and the container are measured.
The measurement should meet the requirements of the assertion policies.
However, the hardware attestation report, if any, is not returned.
The Relying Parties could only trust the results in the attestation token from GCA, without verification.

The loading time measurements are conducted by the vTPM, which is not accessible to the Relying Parties.
Apart from the two static images, the measurements also include logs from Shielded VM~\cite{googleShieldedVM} measured boot, loaded kernels as well as environment properties for the \ac{CVM} and the container.

Similar to Section~\ref{sec:gcp:amd}, runtime measurements are impossible.

The Relying Parties could not read the original attestation reports from the hardware.
Instead, they could retrieve the attestation tokens from GCA via HTTP, within the workload.
}

\paragraph{Trusted Computing Base}

The \ac{TCB} is composed of the \ac{SP} firmware, guest firmware, guest OS, and the container image.
Both the guest firmware and the guest OS are provided by GCP and closed source.
The container image could be hosted at public repository, thus verifiable if measured and reported.
The attestation requires the GCP provided vTPM, violating our trust model and additionally, the actual attestation process is outsourced to the GCA service, which again requires implicit trust in Google.
Customising the \ac{TCB} is limited to the containerised application.

\paragraph{Conclusion}

As mentioned in Section~\ref{sec:threatmodel}, our threat model considers the cloud providers as untrusted.
Therefore, the Confidential Space offering cannot provide any assurances for the following reasons:
\begin{itemize}
    \item No access to the \ac{HRoT} directly.
    \item The hardware attestation is completely outsourced to Google. Implicit trust is therefore required.
    \item Due to the usage of AMD \ac{SEV} no integrity protection is provided.
\end{itemize}

==> evaluation/paper.tex <==
\subsection{Papers - Jana \& Tian - 3 pages}

List of all papers we found and selection of papers based on the following criteria in Table~\ref{tab:papers}.

The criteria for selection are:
\begin{itemize}
    \item AMD SEV / Intel SGX only
    \item full attestation framework 
    \item actually used by products OR if a paper contains a novel idea, which seems to be promising for future developments 
    \item open source, as we will evaluate the work from a practical point of view
\end{itemize}

%\input{evaluation/paper_list}

\subsubsection{Veracruz~\cite{brossard2023private}}
% AWS https://github.com/veracruz-project/veracruz

Identity Establishment:
\begin{itemize}
    \item 
\end{itemize}

Metrics:
\begin{itemize}
    \item 
\end{itemize}

Interaction:
\begin{itemize}
    \item 
\end{itemize}

TCB:
\begin{itemize}
    \item 
\end{itemize}


\subsubsection{Parma~\cite{johnson2024confidential}}
Parma~\cite{johnson2024confidential}
% Azure https://github.com/microsoft/hcsshim/tree/main/pkg/securitypolicy
- execution of container group inside VM-based TEE
- AMD SEV-SNP
- execution policies: policies are part of attestation report at UVM initialisation. Provided by customer, describes wich actions are allowed
- container file system: ordered sequence of layers, each layer is verified with dm-verity root hash and must match policy value
- UVM, OS, guest agent measured and can be requested by containers
- attestation: OS, guest agent, configuration with policy
- 

\subsubsection{GuaranTEE~\cite{morbitzer2023guarantee}}
% Azure https://github.com/Fraunhofer-AISEC/guarantee-code/
GuaranTEE~\cite{morbitzer2023guarantee} aims to provide control flow attestation for Intel SGX in untrusted cloud environments. Control Flow Attestation allows a verifier to detect malicious behaviour based on the execution path of a target by comparing it to the expected control flow path. In their approach, two TEEs, target and verifier, run on the same virtual machine. The verifier receives control-flows from the target via a trampoline. A remote verifier can retrieve the logs from the local verifier, showing the complete control flow of the target.

Identity Establishment:
\begin{itemize}
    \item 
\end{itemize}

Metrics:
\begin{itemize}
    \item 
\end{itemize}

Interaction:
\begin{itemize}
    \item 
\end{itemize}

TCB:
\begin{itemize}
    \item 
\end{itemize}

\subsubsection{Integrating TPMs into Firecracker~\cite{parkegren2023trust}}
% AWS https://github.com/DATX05-CSN-8/fctpm-2023/tree/paper

\subsubsection{SPIRE~\cite{pontes2023attesting}}
% https://github.com/ufcg-lsd/spire-amd-sev-snp-node-attestor

\subsubsection{Keylime~\cite{schear2016bootstrapping}}

\subsubsection{Nitriding~\cite{winter2022framework}}
% AWS https://github.com/brave/nitriding-daemon

\subsubsection{Decentralized Trust~\cite{zhang2024teamwork}}
% https://sites.google.com/view/janus-ra

\subsubsection{Multi-Enclave~\cite{zum2021securing}}
% https://github.com/euc2021paper163/MECT



==> evaluation/paper_list.tex <==
\begin{table*}[htb]
\centering
\begin{tabular}{| p{1cm} | p{9cm} | p{2cm} | p{2cm} | p{1.5cm} |}
    \hline 
    \textbf{Paper} & \textbf{Main Contribution} & \textbf{Attest. Framework?} & \textbf{Product?} &  \textbf{Include in Survey} \\
    \hline 
    Antonino et al.\cite{antonino2023flexible} & Protocol for flexible attestation of SEV & no & &  no \\
    \hline
    Brasser et al.\cite{brasser2022trusted} & TCX: architecture for secure container deployment on untrusted cloud (AMD SEV, Kata Containers) & yes & Sanctuary &  no, not open source \\
    \hline
    Brossard et al.\cite{brossard2023private} & framework for computations among a group of mutually distrusting parties & yes & Veracruz & yes \\
    \hline
    Chen et al.\cite{chen2019opera} & OPERA: SGX attestation without using Intel's attestation service & & & yes? git inactive \\
    \hline
    Delignat et al.\cite{delignat2023should} & survey & & & related work \\
    \hline
    Felsen et al.\cite{felsen2019secure} & Secure Function Evaluation using Intel SGX & no & & no \\
    \hline
    Galanou et al.\cite{galanou2023trustworthy} & architecture for attesting web-based services running on TEEs as a user & no & no & no \\
    \hline
    Ge et al.\cite{ge2022hecate} & L1 hypervisor inside a confidential VM & no, TEE framework & & no \\
    \hline
    Gregor et al.\cite{gregor2020trust} & service for trust management in untrausted environments with Byzantine stakeholders & & SCONE &  no, not open source \\
    \hline
    Jia et al.\cite{jia2022hyperenclave} & process-based TEE & no, TEE framework & & no \\
    \hline
    Johnson et al.\cite{johnson2024confidential} & Parma: container attestation and execution integrity based on attested execution policies & & Azure & yes \\
    \hline
    Menetrey et al.\cite{menetrey2022attestation} & survey - review of remote attestation principles & & & related work\\
    \hline
    Morbitzer et al.\cite{morbitzer2023guarantee} & control-flow attestation & & no & yes? \\
    \hline
    Narayana et al.\cite{narayanan2023remote} & virtual TPM that virtualises the hardware root of trust with an untrusted cloud provider & & & yes? \\
    \hline
    Niemi et al.\cite{niemi2022towards} & survey & & & related work \\
    \hline
    Ott et al.\cite{ott2023universal} & universal, hardware-agnostic device-identity and attestation framework & & & yes \\
    \hline
    Ozga et al.\cite{ozga2021triglav} & Triglav: protocol for attesting VM's runtime integrity & yes & SCONE? & not open source? \\
    \hline
    Paju et al.\cite{paju2023sok} & SoK of TEE usage & & & related work \\
    \hline
    Parkegren et al.\cite{parkegren2023trust} & TPM support in Firecracker & & uses Firecracker & yes \\
    \hline
    Parno et al.\cite{parno2010bootstrapping} & introduction to trusted computing & & & background? \\
    \hline
    Pecholt et al.\cite{pecholt2022cocotpm} & CoCoTPM: TPM for VMs in confidential computing (AMD SEV, SEV-SNP) using Confidential Containers & & & no? \\
    \hline
    Perez et al.\cite{perez2006vtpm} & virtual TPM & no & no & no \\
    \hline
    Pontes et al.\cite{pontes2023attesting} & plugin for attestaion of AMD SEV-SNP & yes & SPIRE & yes? \\
    \hline
    Pop et al.\cite{pop2022towards} & enclave software based on WASM for secure migration & no, TEE migration & & no? \\
    \hline
    Schear et al.\cite{schear2016bootstrapping} & bootstrapping hardware rooted cryptographic identities in IaaS cloud & yes & Keylime & yes \\
    \hline
    Scopelliti et al.\cite{scopelliti2024understanding} & survey - attestability of TEE hardware and CVM stack & & & related work \\
    \hline
    Segarra et al.\cite{segarra2024serverless} & port of Knative serverless runtime to Confidential Containers & no & CoCo & no \\
    \hline
    Sfyrakis et al.\cite{sfyrakis2020survey} & survey - remote attestation in network infrastructures & & & related work \\
    \hline
    Winter et al.\cite{winter2022framework} & open tool kit for development of enclave applications & AWS Nitro & & yes \\
    \hline
    Zhang et al.\cite{zhang2024teamwork} & decentralised trust establishment by using PUF as additional RoT & & & yes \\
    \hline
    Zum et al.\cite{zum2021securing} & multi-enclave architecture for remote enforcement of usage control & & & no? \\
    \hline 
\end{tabular}
\caption{Research Papers}
\label{tab:papers}
\end{table*}

==> evaluation/questions.tex <==
\subsubsection{Questions to be answered}

What is the TCB for setting up a TEE instance? 
\begin{enumerate}
    \item Can the TCB be configured?
    \item Can it be validated? 
\end{enumerate}

Can we retrieve and individualize an attestation report? 
\begin{enumerate}
    \item Who owns the different layers/components used to configure and produce the report?
    \item Are these components open source and can be validated or closed and what entity do we have to trust in that case?
    \item Who is the root of trust for the report? Is there a trust chain of different entities? (e.g., hardware vendor, cloud provider etc.)
    \item Can the customer provision a different root of trust or trust chain?
    \item What exactly is covered by the measurement of the attestation report?
Example: HW/SW of CPU provider, customer code/data, cloud provider SW/HW
    \item Is there additional data that can be included/linked into the report?
Example: Data provided by the TEE protected SW, additional data provided during setup (customer, developer and provider)
    \item Are the communication paths to create an attestation report integrity-protected and secure? Which components are involved? 
\end{enumerate}
